Characterization of the scintillation anisotropy in crystalline stilbene scintillator detectors

This paper reports a series of measurements that characterize the directional dependence of the scintillation response of crystalline melt-grown and solution-grown stilbene to incident DT and DD neutrons. These measurements give the amplitude and pulse shape dependence on the proton recoil direction over one hemisphere of the crystal, confirming and extending previous results in the literature for melt-grown stilbene and providing the first measurements for solution-grown stilbene. In similar measurements of liquid and plastic detectors, no directional dependence was observed, confirming the hypothesis that the anisotropy in stilbene and other organic crystal scintillators is a result of internal effects due to the molecular or crystal structure and not an external effect on the measurement system.

==> general.tex <==
\FloatBarrier % Don't let any graphics from the previous section leak into this one
\chapter{Some General Stuff to Keep Around}

% Websites with good tips
% http://thewanderingengineer.com/2015/06/23/latex-tips-and-tricks-for-thesis-writing/

\section*{Figures}
I'm going to put lots of pictures in this paper. Starting with a missing one in \fig{fig:ImageHere}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Missing Figure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% trim={<left> <lower> <right> <upper>}
% MATLAB default lengths: https://en.wikibooks.org/wiki/LaTeX/Lengths
\begin{figure}
	\centering
	\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=.33\textwidth]{fig/ImageHere.pdf}
	\caption{I will put a picture here someday.
	\label{fig:ImageHere}
	}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Subfigures}
I should also have some missing subfigures too in \fig{fig:ImageHere1} and \fig{fig:ImageHere2}. Together they make \fig{fig:ImageHereSubFig}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Missing Subfigure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% trim={<left> <lower> <right> <upper>}
% MATLAB default lengths: https://en.wikibooks.org/wiki/LaTeX/Lengths
\begin{figure}[!t]
	\centering
	\subfloat[First missing image.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=2.5in]{fig/ImageHere.pdf}%
		\label{fig:ImageHere1}}
	\hfil
	\subfloat[Second missing image.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=2.5in]{fig/ImageHere.pdf}%
		\label{fig:ImageHere2}}
	\caption{Two missing images.}
	\label{fig:ImageHereSubFig}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

And if I want to have three missing subfigures in \fig{fig:ImageHere3}, \fig{fig:ImageHere4} and \fig{fig:ImageHere5}, I can set them up so they make \fig{fig:ImageHereSubFigs}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Missing Subfigure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% trim={<left> <lower> <right> <upper>}
% MATLAB default lengths: https://en.wikibooks.org/wiki/LaTeX/Lengths
\begin{figure}[!t]
	\centering
	\subfloat[First missing image.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=2.5in]{fig/ImageHere.pdf}
		\label{fig:ImageHere3}}
	\hfil
	\subfloat[Second missing image.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=2.5in]{fig/ImageHere.pdf}%
		\label{fig:ImageHere4}}
	\hfil
	\subfloat[Third missing image.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=2.5in]{fig/ImageHere.pdf}%
		\label{fig:ImageHere5}}
	\caption{Two missing images.}
	\label{fig:ImageHereSubFigs}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section*{Equations}
I also want to include a lot of equations, like \eqnref{eqn:general}. And I want to align them like in \eqnref{eqn:general}. If there is too much spacing when using \verb|align|, use \verb|alignat*| like in \eqnref{eqn:general3}
%%%%%%%%%%%%%%%%%%%%%%% EQUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}\label{eqn:general}
	y = mx + b
\end{equation}
% If I want to line up the equations, use align*
% If I want to number an equation in align* and reference it
\begin{align*}
y &= mx+b \\
z &= my+c \numberthiseqn \label{eqn:general2}
\end{align*}
% Prevent it from spreading out- argument at end is number of columns
\begin{alignat*}{2}
y &= mx+b \\
z &= my+c \numberthiseqn \label{eqn:general3}
\end{alignat*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\note{Here's a note to myself}
\todo{do this later}
\missref{this paper}
\rephrase{Rephrase this section}

\section*{Lists}
To make a numbered list, use \verb|enumerate|:
\begin{enumerate}
	\item First item
	\begin{enumerate}
		\item First subitem
		\item Second subitem		
	\end{enumerate}
	\item Second item
\end{enumerate}

To make a bulleted list, use \verb|itemize| without any options. To make the list more compact, use \verb|noitemsep| from the \verb|enumitem| package:
\begin{itemize}[noitemsep]
	\item First item
	\begin{itemize}[noitemsep]
		\item First subitem
		\item Second subitem		
	\end{itemize}
	\item Second item
\end{itemize}

To change the bullet type in an \verb|itemize| list, either change it item by item, or for the whole list.
\begin{itemize}[noitemsep]
	\item Two items below have the same special symbol
	\begin{itemize}[noitemsep,label={--}]
		\item First subitem
		\item Second subitem		
	\end{itemize}
	\item[*] Item with unique symbol
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%% ITEMIZED LIST %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
My general format for an itemized list will look like this:
\begin{itemize}[noitemsep,label={--}]
	\item Item 1
	\item Item 2
	\item Item 3
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Managing and citing references}
Time to cite a paper. How I create my references (and how I make a numbered list):
\begin{enumerate}
	\item Open Mendeley
	\item Highlight all documents to reference (easiest is just to select everything in my library)
	\item Right click $\rightarrow$ ``Export..."
	\item Save as ``...Google Drive/Resources/Mendeley/Archive/yyyy\_mm\_dd\_references.bib"
	\item Copy latest version to LaTeX folder 
	\item Call it in LaTeX main file with \verb|\bibliography{yyyy_mm_dd_references}|
\end{enumerate}

\textbf{Cite a paper:} To cite the entire paper, use \verb|\cite{Akselrod2014}| to produce this type of reference: \cite{Akselrod2014}.

\textbf{Cite a book:} To cite the entire book, use \verb|\cite{Birks1964}| to produce this type of reference: \cite{Birks1964}.

\textbf{Citing a chapter in a book:} To cite a chapter in a book, use \verb|\cite[ch.~4]{Birks1964}| to produce this type of reference: \cite[ch.~4]{Birks1964}. Similar process for citing a range of page numbers.


\section*{Importing code from other works}
I am going to write a function called \verb|\directcopy{#1,#2}| for when I copy large chunks of other papers into my thesis. This way, it will be highlighted as a section that needs to be updated. As an example:

\directcopy{Anthracene Paper}{Here is my Anthracene paper.}

Figure definitions may be included as argument \verb|#2| in \verb|\directcopy{#1,#2}|, but I recommend they are placed outside of the command. \verb|\directcopy{#1,#2}| is meant for full paragraphs of text that need to be moved around or reorganized. References or citations included in argument \verb|#2| will work.

If I want to display raw MATLAB code, use this:
\begin{lstlisting}[style=Matlab-editor,frame=single]
function m = myfunc(x,y)
\end{lstlisting}
